Modeling Epistemological Principles for Bias Mitigation in AI Systems: An Illustration in Hiring Decisions

Artificial Intelligence (AI) has been used extensively in automatic decision making in a broad variety of scenarios, ranging from credit ratings for loans to recommendations of movies. Traditional design guidelines for AI models focus essentially on accuracy maximization, but recent work has shown that economically irrational and socially unacceptable scenarios of discrimination and unfairness are likely to arise unless these issues are explicitly addressed. This undesirable behavior has several possible sources, such as biased datasets used for training that may not be detected in black-box models. After pointing out connections between such bias of AI and the problem of induction, we focus on Popper's contributions after Hume's, which offer a logical theory of preferences. An AI model can be preferred over others on purely rational grounds after one or more attempts at refutation based on accuracy and fairness. Inspired by such epistemological principles, this paper proposes a structured approach to mitigate discrimination and unfairness caused by bias in AI systems. In the proposed computational framework, models are selected and enhanced after attempts at refutation. To illustrate our discussion, we focus on hiring decision scenarios where an AI system filters in which job applicants should go to the interview phase.

==> includes/optimization.tex <==
% !TEX root = ../paper.tex

\section{Lakatosian approach to improvements in machine learning models}


Popper's falsificationism suggests the elimination of a theory or model once a counter-example showing its falsehood has been identified \cite{popper1935logik}. This concept has been applied in science since its conception, and, in particular, it fits well the definition employed in computer science for the concept of algorithms, specially if deterministic problems are being considered. For instance, a procedure that fails to provide the correct solution for any input of the problem is not considered an algorithm, but a heuristic (or an approximation algorithm in case some bound on the distance between the optimal solution and the one provided by the procedure is known). 



For algorithms based on statistical learning, though, there are several challenges involved on the application of falsificationism. Corfield, Sch\"{o}lkopf, and Vapnik compare Popper's ideas with the theory of statistical learning~\cite{corfield2005popper}. In particular, the authors compare the VC-dimension, proposed by Vapnik and Chervonenkis~\cite{vapnik2013nature}, with Popper's dimension of a theory (this comparison was also presented by Seldin and  Sch{\"o}lkopf~\cite{seldin2013relations}). From this analysis, the authors conclude that either Popper was not sufficiently precise enough in his definitions (similar discussions have been presented in the literature; see e.g., \cite{turney1991note}), or that the goals he had for his theory were focused in scenarios where the discovery process was more focused on the identification of issues in a theory rather than on its reliability, expressiveness, and accuracy level.




First, error and noise are inherent to algorithms and models based on statistical learning, so falsification in this context will typically involve more than strange results for a single input. Additionally, problems with infinite (or even sufficiently large) domains impose a severe constraint on the assessment of  models; namely, the enumeration and verification of  all possible inputs is unpractical or even impossible, thus restricting the application of exhaustive search methods for validation. Finally, the accuracy reached by state-of-the-art algorithms  may be sufficiently large to compensate for eventual mistakes they might make. 

For these reasons, the concept or \marisa{DEFINIR: research programs} proposed by Lakatos seems to provide the most adequate philosophical framework guiding the formulation, development, and adjustment of models generated by machine learning methods~\cite{lakatos2014falsification}. In summary, Lakatos proposes a methodology in which a series of hypotheses or axioms constitute a \textit{hard core}, which should not be subject to changes, and several \textit{auxiliary hypotheses},  which can be interpreted as ``local adjustments'' to support or complement the hard core. Under this framework, falsificationism is used to support the refinement and further development of a theory. A trade-off between expressiveness and correctness apply in these cases: namely, the incorporation of hypotheses increase the level of control over the environment and therefore potentially increase the accuracy with which the problem at hand is represented, but these gains are obtained at the expense of a lesser level of generality.

In the context of machine learning models, a research program may be supported by frameworks responsible for the identification of bias, disparate treatment, fairness, and other elements that may provide sufficient a relatively structured approach to tackle confirmation bias. 
% \marisa{Acho que nao eh tanto identificacao de bias, mas evitar disparate treatment e impact que caracterizam o comportamento discriminatorio}. 
ßIn particular, this approach would suit well models whose construction are based on constraint optimization formulations of the problem at hand. Constrained optimization models are ubiquitous in operations research (REFERENCIAS?). One can also observe examples in machine learning (REFERENCIAS?). The incorporation of constraints to machine learning models in order to eliminate or bound the amount of bias they may yield has been proposed in the literature already; for instance, Zafar et al. recently proposed classifiers using convex optimization that maximize accuracy while respecting predefined fairness constraints~\cite{zafar2017fairness}.

Straightforward modeling techniques in optimization rely on a full formal characterization of the problem at hand. Namely, all constraints must be known a priori and the formulation must be succinct enough to fit in a computer's main memory. In cases where such a formulation is possible, the research program is more closely related to Popper's falsificationism approach, in the sense that wrong or undesirable outputs may result in the necessity for a new formulation, where constraints are included, removed, changed, or even fixed. Research programs relying on this approach are more likely to have a slower progress, as model refinements will necessarily involve human interaction.


In many cases, though, the number of constraints required for a complete representation of the problem is too large for explicit enumeration. This is typically the case of formulations whose dimensions is exponential in the size of the problem. In mathematical programming and optimization, several (iterative) solution techniques have been proposed in order to overcome this challenge. In particular, procedures based on the generation of cuts have an interesting connection with the Lakatosian approach to machine learning models discussed in this section. In a typical cut-generation algorithm, one does not work with a complete formal representation of the problem at hand, but with a simplification (or relaxation), in which certain constraints and conditions are not included in the current model. By construction, every feasible solution of the original problem is associated with a feasible solution for the relaxed model. Conversely, feasible solutions for the relaxed model may not be acceptable for the original model; whenever such a solution is generated, a cut-generation procedure is employed in order to generate one or more inequalities that will typically preserve the validity of all feasible solutions for the original problem while removing a current solution presenting some undesirable property.

A Lakatosian research program for machine learning models resembles optimization approaches based on relaxation and cut-generation  under several perspectives. First, problems addressed by machine learning algorithms are typically not amenable to a complete formal characterization; in short, they do not have sufficient structure allowing for succinct and exact representation of their solution space. Therefore, machine learning models can be interpreted as relaxations of a more comprehensive model that may not be achievable. The identification of bias and the creation of auxiliary hypotheses based on this knowledge in order to strengthen the current formulation is equivalent to the cut-generation procedure. 

An obvious critic about such approaches would be the impossibility to have a complete model, capable of capturing all the details that a problem would require. The same argument applies to optimization models, though, and classical results in the area show that this restriction is not critical in several important scenarios. For instance, the celebrated theorem of Gr\"{o}tschel, Lov\'{a}sz, and Schrijver show that an efficient (polynomial-time) procedure for inspecting the pertinence of a vector in a convex set~$K$ allows for the efficient optimization of any linear function over~$K$~\cite{grotschel2012geometric}. In other words, if cuts can be generated efficiently, a problem can be optimized in polynomial time. 

Strong results and techniques such as the ones enabled by the Gr\"{o}tschel-Lov\'{a}sz-Schrijver theorem rely on very strong requisites; for instance, convexity is a crucial hypothesis for this result. Some efforts in the area of optimization and logic inference, though, show that these ideas may be applied in more general frameworks. Particularly interesting is the work of Hooker and Ottosson, in which logic-based Benders decomposition method is introduced~\cite{hooker2003logic}. The original Benders decomposition method relies on strong assumptions about the problem at hand (namely, the dual problem should be a linear program), and later extensions were also restrictive in terms of the classes of problems that could be addressed~\cite{benders1962partitioning,geoffrion1972generalized}. Hooker and Ottosson showed that the same idea for any optimization problem if problem-specific logic inference techniques are applied.
 

A research program based solely on falsificationism related with bias is not comprehensive, in the sense that a completely bias-free model is not necessarily perfect or even satisfactory for the problem at hand. Nevertheless, the identification of certain types  of bias is relatively easy, making a bias-free-driven approach to model sophistication achievable.

\marisa{Duvida: Vc estah tentando identificar o bias ou criar um comportamento nao discriminatorio no seu algoritmo? O quanto essas abordagem sao aplicadas aos algoritmos mais populares de ML?}

pontos a considerar/ajustar:
\begin{itemize}
	\item Popper fala que universal statements \textbf{with infinite domains} can be falsified but not verified
	\item According to Vapnik, Popper's theory is not expressive enough to evaluate the reliability of well-tested theories.
\end{itemize}


